Fibredness of 3-manifolds is in NP

We show that the problem of deciding whether a compact orientable 3-manifold fibres over the circle lies in the complexity class NP.

==> interval-bundles.tex <==
\section{Topology of interval bundles}

\subsection{Essential surfaces in interval bundles}

\begin{proposition}[Essential surfaces in interval bundles are vertical]
\label{thm:essential surfaces in interval bundles are vertical}
Let $M=F\times[0,1]$ for some compact orientable surface $F$, and consider the boundary pattern $\Gamma=\boundary F\times\{0,1\}$.
Let $A$ be a surface properly embedded in $(M,\Gamma)$ that is incompressible and boundary\=/incompressible.
Suppose that no component of $A$ is a surface without boundary or a disc intersecting $\Gamma$ at most twice, and that no component of $\boundary A$ is contained in $\vboundary M$.
Then $A$ is vertical in $M$.
\end{proposition}
\begin{proof}
We can assume without loss of generality that $A$ is connected, and moreover that $M$ is connected.
If any component of $A\cap\vboundary M$ is an arc with both endpoints on $\boundary_0 M$ or $\boundary_1 M$, then we immediately see that $A$ is boundary\=/compressible.
Therefore, every component of $A\cap\vboundary M$ is a vertical arc.

We now wish to invoke \cite[Proposition~5.6]{johannson:homotopy-equivalences-3} to conclude that $A$ must be vertical.
To this aim, we must first translate the definition of ``essential'' from \cite[Definition~3.1]{johannson:homotopy-equivalences-3} to our setting.
We say that a surface $S$ properly embedded in $(M,\Gamma)$ is \emph{essential in the sense of \cite{johannson:homotopy-equivalences-3}} if
\begin{itemize}
\item $S$ is incompressible in $M$, and
\item for any (not necessarily clean) boundary\=/compressing disc $D$ for $S$ in $M$ that intersects $\Gamma$ at most once, the arc $D\cap S\subs S$ cuts a disc off of $S$ that intersects $\Gamma$ at most once.
\end{itemize}
Then \cite[Proposition~5.6]{johannson:homotopy-equivalences-3} implies the following: if $F$ is not a sphere nor a disc, then any surface $S$ properly embedded in $(M,\Gamma)$ that is essential in the sense of \cite{johannson:homotopy-equivalences-3} is horizontal or vertical in $M$, provided that no component of $S$ is a sphere or a disc intersecting $\Gamma$ at most three times; in fact, ``three'' can be replaced by ``two'' here, since $S$ will necessarily intersect $\Gamma$ an even number of times.
Note that, if $F$ were a sphere or a disc, then $A$ would necessarily be compressible or boundary\=/compressible.
Moreover, the surface $A$ cannot be horizontal, because $\boundary A$ intersects $\hboundary M$ by assumption.

Therefore, all we need to show is that $A$ is essential in the sense of \cite{johannson:homotopy-equivalences-3}.
We already know that $A$ is incompressible in $M$.
Let $D$ be a boundary\=/compressing disc for $A$ in $M$ that intersects $\Gamma$ at most once.
If $D$ is clean, then by boundary\=/incompressibility of $A$ we know that $D\cap A$ cuts a clean disc off of $A$.
Otherwise, the boundary of $D$ is naturally split into three non\=/empty arcs: let $a=D\cap A$, $b_v=D\cap\vboundary M$, and $b_0=D\cap\hboundary M$.
Without loss of generality, assume that $b_0\subs\boundary_0 M$.
Let $c$ be the subarc of $A\cap\vboundary M$ that connects an endpoint of $b_v$ to $\boundary_0 M$; the existence of such a subarc is guaranteed by our previous observation that every component of $A\cap\vboundary M$ is a vertical arc.
This situation is depicted in \zcref{fig:essential surfaces in interval bundles are vertical:a}.

The arc $b_v\cup c$ cuts a disc $D_v$ off of $\vboundary M$.
The disc $D\cup D_v$ can be isotoped slightly off of $\vboundary M$ to a clean boundary\=/compressing disc $D'$ for $A$.
Since $A$ is boundary\=/incompressible, we deduce that the arc $D'\cap A$ cuts a clean disc off of $A$.
It is then easy to conclude (see \zcref{fig:essential surfaces in interval bundles are vertical:b}) that $a$ cuts a disc off of $A$ that intersects $\Gamma$ exactly once -- in particular, the point of intersection is $\boundary c_v\setminus b_v$.
This concludes the proof, since $A$ is essential in the sense of \cite{johannson:homotopy-equivalences-3} and therefore vertical in $M$.\qedhere

\begin{myfigure}
\begin{subfigure}{0.45\textwidth}
\centering
\myfiguresource[scale=.3]{essential-surfaces-in-interval-bundles-are-vertical-a}
\caption{}
\label{fig:essential surfaces in interval bundles are vertical:a}
\end{subfigure}\hfill
\begin{subfigure}{0.45\textwidth}
\centering
\myfiguresource[scale=.3]{essential-surfaces-in-interval-bundles-are-vertical-b}
\caption{}
\label{fig:essential surfaces in interval bundles are vertical:b}
\end{subfigure}
\caption{\subref{fig:essential surfaces in interval bundles are vertical:a} The boundary\=/compressing disc $D$ for $A$ intersects $\Gamma$ at most once.
\subref{fig:essential surfaces in interval bundles are vertical:b} The disc $D\cup D_v$ can be isotoped to a clean boundary\=/compressing disc $D'$ for $A$.}
\end{myfigure}
\end{proof}

\subsection{Triangulations of interval bundles}
It should come as no surprise that the minimum number of tetrahedra needed to triangulate an interval bundle over a planar surface $F$ is linear in the number of boundary components of $F$.
For our fibredness certificate, we will need a more refined version of this estimate, that asks how many tetrahedra are needed to extend a given triangulation of a vertical subset of $\boundary F\times[0,1]$ to a triangulation of $F\times[0,1]$.
The answer turns out to be linear in the number of triangles of the prescribed triangulation, provided that the vertical subset touches every component of $\boundary F\times[0,1]$.

\begin{proposition}[Triangulating interval bundles over planar surfaces efficiently]
\label{thm:triangulating interval bundles efficiently}
Let $M=F\times[0,1]$ for some compact orientable planar surface $F$.
Let $\Omega\subs\boundary F$ be a union of finitely many circles or closed intervals with non\=/empty interiors; suppose that $\Omega$ intersects every component of $\boundary F$.
Let $\TTT_0$ be a triangulation of $\Omega\times[0,1]\subs\vboundary M$ with $t_0$ triangles, such that every point in $\boundary\Omega\times\{0,1\}$ is a vertex of $\TTT_0$.
Then there is a triangulation $\TTT$ of $M$ such that:
\begin{enumarabic}
\item the restriction of $\TTT$ to $\Omega\times[0,1]$ is $\TTT_0$;
\item the restriction of $\TTT$ to $\hboundary M$ is flapless;
\item the number of tetrahedra of $\TTT$ is at most $26t_0$.
\end{enumarabic}
\end{proposition}
\begin{proof}
It is not restrictive to assume that $M$ is connected.
We start by finding a triangulation $\TTT_1$ of $\vboundary M$ that agrees with $\TTT_0$ on $\Omega\times[0,1]$.
Denote by $b_1,\dots,b_m$ the components of $\boundary F$; for each $1\le i\le m$, we construct a triangulation of $b_i\times[0,1]$.
Let $\Omega_i=\Omega\cap b_i$, and let $s_i$ be the number of triangles of $\TTT_0$ contained in $\Omega_i\times[0,1]$.
If $b_i\subs\Omega$, then we simply triangulate $b_1\times[0,1]$ by restricting $\TTT_0$.
Otherwise, denote by $k$ the number of components of $\Omega_i$, and by $h$ the number of edges of $\TTT_0$ that are contained in $\boundary\Omega_i\times[0,1]$; a simple counting argument shows that $s_i\ge h$.
The closure of the complement of $\Omega_i\times[0,1]$ in $b_i\times[0,1]$ is a union of topological discs; each of these discs has a natural cell structure of its boundary, with one edge on $b_i\times\{0\}$, one on $b_i\times\{1\}$, and the remaining edges on $\boundary\Omega_i\times[0,1]$ coming from $\TTT_0$.
The number of these discs is $k$, and the combined simplicial length of their perimeters is exactly $2k+h$.
Therefore, their union can be triangulated with exactly $h$ triangles, as shown in \zcref{fig:triangulating interval bundles efficiently:triangulating vboundary}.

\begin{myfigure}

\myfiguresource[scale=.3]{triangulating-interval-bundles-efficiently-triangulating-vboundary}
\caption{The triangulation $\TTT_1$ restricted to $b_i\times[0,1]$.
The edges and triangles of $\TTT_1$ that are not in $\TTT_0$ are highlighted.}
\label{fig:triangulating interval bundles efficiently:triangulating vboundary}
\end{myfigure}

In conclusion, we have constructed a triangulation of $b_i\times[0,1]$ with at most $2s_i$ triangles (recall that $h\le s_i$) that agrees with $\TTT_0$ on $\Omega_i\times[0,1]$.
Repeating this construction for every boundary component $b_i$ yields a triangulation $\TTT_1$ of $\vboundary M$ that agrees with $\TTT_0$ on $\Omega\times[0,1]$ and has
\begin{equation}\label{eqn:triangulating interval bundles efficiently:t1}
t_1\le2s_1+\dots+2s_m=2t_0
\end{equation}
triangles.

The next step is to find a triangulation of a union $S$ of squares in $M$ that agrees with $\TTT_1$ on $S\cap\vboundary M$, such that $M\cut S$ is a $3$\=/ball.
To this aim, for each $1\le i\le m$, fix a simplicial arc $a_i\subs b_i\times[0,1]$ that is vertical in $M$.
Denote by $\ell_i$ the simplicial length of $a_i$, and -- without loss of generality -- assume that $\ell_1\le\ell_i$ for every $2\le i\le m$.
Find squares $S_2,\dots,S_m$ in $M$ such that $S_i\cap\vboundary M=a_1\cup a_i$ for each $2\le i\le m$, and $S_i\cap S_j=a_1$ for all $1\le i<j\le m$.
The boundary of each $S_i$ has a natural cell structure with exactly $\ell_1+\ell_i+2$ edges; therefore, we can triangulate $S_i$ with $\ell_1+\ell_i$ triangles.
Let $\TTT_2$ be the triangulation of $S=S_2\cup\dots\cup S_m$ obtained from this construction, as shown in \zcref{fig:triangulating interval bundles efficiently:S}. The number $t_2$ of triangles of $\TTT_2$ is exactly
\begin{equation}\label{eqn:triangulating interval bundles efficiently:t2}
t_2=(m-1)\ell_1+\ell_2+\dots+\ell_m.
\end{equation}

Finally, we construct a triangulation of $M$, by exploiting the fact that $B=M\cut S$ is a topological $3$\=/ball.
The triangulations $\TTT_1$ and $\TTT_2$ induce a cell structure on the boundary of $B$, consisting of $t_1+2t_2$ triangles and two polygons $P_0$ and $P_1$, where $P_i=B\cap\boundary_i M$ for $i\in\{0,1\}$; this is depicted in \zcref{fig:triangulating interval bundles efficiently:B}.
Note that, for each $i\in\{0,1\}$, the number of edges of $P_i$ is exactly $r_i+2m-2$, where $r_i$ is the number of edges of $\TTT_1$ that are contained in $\boundary_i M$.
We can then triangulate each $P_i$ with $r_i+2m-2$ triangles, by coning over a point in the interior of $P_i$; this construction guarantees that the triangulation of each $P_i$ is flapless, and it produces a triangulation of $\boundary B$ with exactly
\[
t_1+2t_2+r_0+r_1+4m-4
\]
triangles.
By coning over a vertex of $B$, we obtain a triangulation $\TTT_3$ of $B$ whose number $t_3$ of tetrahedra is at most
\begin{equation}\label{eqn:triangulating interval bundles efficiently:bound on t3}
t_3\le t_1+2t_2+r_0+r_1+4m-5.
\end{equation}
We conclude by gluing this triangulation of $B$ along $S$ to obtain a triangulation $\TTT$ of $M$.

\begin{myfigure}
\begin{subfigure}[b]{.42\linewidth}
\centering
% \myfiguresource[scale=.3]{triangulating-interval-bundles-efficiently-S}
\caption{}
\label{fig:triangulating interval bundles efficiently:S}
\end{subfigure}\hfill
\begin{subfigure}[b]{.48\linewidth}
\centering
% \myfiguresource[scale=.3]{triangulating-interval-bundles-efficiently-B}
\caption{}
\label{fig:triangulating interval bundles efficiently:B}
\end{subfigure}
\caption{\subref{fig:triangulating interval bundles efficiently:S} For each $2\le i\le m$, the square $S_i$ can be triangulated with $\ell_1+\ell_i$ triangles. \subref{fig:triangulating interval bundles efficiently:B} The topological $3$\=/ball $B=M\cut S$ has a natural cell structure, consisting of triangles coming from $\TTT_1$ and (two copies of) $\TTT_2$, and two polygons $P_0$ and $P_1$.}
\end{myfigure}

By construction, the restriction of $\TTT$ to $\Omega\times[0,1]$ is exactly $\TTT_0$, and the restriction of $\TTT$ to $\hboundary M$ is flapless, so all that is left is bounding the number of tetrahedra of $\TTT$ -- or, equivalently, of $\TTT_3$.
Let $s$ be the number of edges of $\TTT_1$; note that, trivially, we have the bound $s\le 3t_1$.
We also remark that, equally trivially, we have that $r_i\ge m$ for $i\in\{0,1\}$.
Elementary counting arguments show that
\begin{align}
\ell_1+\dots+\ell_m+r_0+r_1&\le s\le 3t_1,
\label{eqn:triangulating interval bundles efficiently:sum of l and r}\\
m\ell_1\le\ell_1+\dots+\ell_m&\le 3t_1-2m.
\label{eqn:triangulating interval bundles efficiently:m times l1}
\end{align}
We can finally bound the number of tetrahedra of $\TTT_3$ as follows:
\begin{alignaside*}
t_3&\le t_1+2t_2+r_0+r_1+4m-5&\aside{by \zcref{eqn:triangulating interval bundles efficiently:bound on t3}}\\
&=t_1+2(m-1)\ell_1+2\ell_2+\dots+2\ell_m+r_0+r_1+4m-5&\aside{by \zcref{eqn:triangulating interval bundles efficiently:t2}}\\
&\le 4t_1+(2m-3)\ell_1+\ell_2+\dots+\ell_m+4m-5&\aside{by \zcref{eqn:triangulating interval bundles efficiently:sum of l and r}}\\
&\le 7t_1+2(m-2)\ell_1+2m-5&\aside{by \zcref{eqn:triangulating interval bundles efficiently:m times l1}}\\
&\le13t_1-4\ell_1-2m-5&\aside{by \zcref{eqn:triangulating interval bundles efficiently:m times l1}}\\
&< 13t_1&\aside{since $\ell_1\ge0$ and $m\ge 0$}\\
&\le 26t_0&\aside{by \zcref{eqn:triangulating interval bundles efficiently:t1}.\qedhere}
\end{alignaside*}
\end{proof}


\subsection{Recognition of interval bundles}
The most basic algorithmic problem about interval bundles asks whether a given triangulated $3$\=/manifold is a product interval bundle over some compact orientable surface.
However, our $3$\=/manifolds often come equipped with information about where the horizontal and vertical boundary of the candidate interval bundle should be -- in other words, with a pre\=/sutured triangulation.
The question we are interested in is then the following.

\begin{algoproblem}[\problemname{Sutured interval bundle recognition}]
\label{prb:interval bundle recognition}
\Input{a pre\=/sutured triangulation $\TTT$ of a compact $3$\=/manifold.}
\Output{whether $\TTT$ is a suitable pre\=/sutured triangulation of $F\times[0,1]$ for some compact orientable surface $F$.}
The size of the input is measured by the number of tetrahedra in $\TTT$.
\end{algoproblem}

It turns out that a positive answer to this question can be certified in polynomial time.

\begin{theorem}[{\nameref{prb:interval bundle recognition} is in \NP}]
\label{thm:interval bundle recognition is in NP}
The problem \nameref{prb:interval bundle recognition} is in \NP{}.
\end{theorem}

This result appears as Theorem 12.1 in \cite{lackenby:efficient-certification-knottedness}, stated in greater generality for handle structures instead of pre\=/sutured triangulations.
In fact, to be precise, since we are given as input a pre\=/sutured triangulation instead of a \emph{sutured triangulation}, a pre\=/processing step is required, to verify that the given pre\=/sutured triangulation is indeed a sutured triangulation.
In practice, for a given pre\=/sutured triangulation of a $3$\=/manifold $M$, one simply needs to check that $\vboundary M$ is a union of annuli, each of which intersects both $\boundary_0 M$ and $\boundary_1 M$; this can be easily carried out in polynomial time in the size of the triangulation.
More crucially, the reader should be aware that the published proof of \cite[Theorem~12.1]{lackenby:efficient-certification-knottedness} contains a gap, in that it only works for sutured triangulations with non\=/empty sutures -- in other words, when the surface $F$ has non\=/empty boundary.
However, this issue can easily be fixed by cutting the $3$\=/manifold along a vertical normal annulus with bounded weight, which can be provided as part of the certificate; this is discussed at the beginning of \cite[Section~11]{lackenby-schleimer:recognising-elliptic-manifolds}.
